What is Wrong with Topic Modeling? (and How to Fix it Using Search-based Software Engineering)

Context: Topic modeling finds human-readable structures in unstructured textual data. A widely used topic modeler is Latent Dirichlet allocation. When run on different datasets, LDA suffers from "order effects" i.e. different topics are generated if the order of training data is shuffled. Such order effects introduce a systematic error for any study. This error can relate to misleading results;specifically, inaccurate topic descriptions and a reduction in the efficacy of text mining classification results. Objective: To provide a method in which distributions generated by LDA are more stable and can be used for further analysis. Method: We use LDADE, a search-based software engineering tool that tunes LDA's parameters using DE (Differential Evolution). LDADE is evaluated on data from a programmer information exchange site (Stackoverflow), title and abstract text of thousands ofSoftware Engineering (SE) papers, and software defect reports from NASA. Results were collected across different implementations of LDA (Python+Scikit-Learn, Scala+Spark); across different platforms (Linux, Macintosh) and for different kinds of LDAs (VEM,or using Gibbs sampling). Results were scored via topic stability and text mining classification accuracy. Results: In all treatments: (i) standard LDA exhibits very large topic instability; (ii) LDADE's tunings dramatically reduce cluster instability; (iii) LDADE also leads to improved performances for supervised as well as unsupervised learning. Conclusion: Due to topic instability, using standard LDA with its "off-the-shelf" settings should now be depreciated. Also, in future, we should require SE papers that use LDA to test and (if needed) mitigate LDA topic instability. Finally, LDADE is a candidate technology for effectively and efficiently reducing that instability.

==> Makefile <==
Src=main#
Bib=$(shell ls *.bib *.bst)#
D=$(HOME)/tmp/$(Src)#
define grab
   gs -sDEVICE=pdfwrite -dNOPAUSE -dBATCH -dSAFER \
       -dFirstPage=$(1) -dLastPage=$(2) \
       -sOutputFile=$@ $<
endef

all: dirs tex bib  tex tex tex     done

typo:
	- git status
	- git commit -am "typo"
	- git push origin master

commit:
	- git status
	- git commit -a
	- git push origin master

update:
	- git pull origin master

status:
	- git status

one: dirs tex done 

open:
	open $(D).pdf

evince:
	evince $(D).pdf 2> /dev/null &


skim:
	/Applications/Skim.app/Contents/MacOS/Skim $(D).pdf &


view:
	evince $(D).pdf &

abe :  $(D)_a.pdf $(D)_b.pdf $(D)_e.pdf

$(D).pdf : $(Src).tex $(Bib)
	pdflatex -output-directory=$(HOME)/tmp $(Src)

$(D)_a.pdf : $(D).pdf; $(call grab,1,1)		
$(D)_b.pdf : $(D).pdf; $(call grab,2,16)		
$(D)_e.pdf : $(D).pdf; $(call grab,18,28)		

done: embedfonts  
	@printf "\n\n\n==============================================\n"
	@printf       "see output in $(D).pdf\n"
	@printf       "==============================================\n\n\n"
	@printf "\n\nWarnings (may be none):\n\n"
	grep arning $D.log

dirs: 
	- [ ! -d $(HOME)/tmp ] && mkdir $(HOME)/tmp

tex: files $(D).pdf

files:
	cp *.tex $(HOME)/tmp

embedfonts:
	@ gs -q -dNOPAUSE -dBATCH -dPDFSETTINGS=/prepress -sDEVICE=pdfwrite \
          -sOutputFile=$(D)-embedded.pdf $(D).pdf
	@ mv  $(D)-embedded.pdf $(D).pdf

bib:
	echo $(Bib)
	- cp $(Bib) $(HOME)/tmp; cd $(HOME)/tmp; bibtex $(Src)
clean:
	rm $D.*

